Contextual Bandits in a Survey Experiment on Charitable Giving: Within-Experiment Outcomes versus Policy Learning

We design and implement an adaptive experiment (a ``contextual bandit'') to learn a targeted treatment assignment policy, where the goal is to use a participant's survey responses to determine which charity to expose them to in a donation solicitation. The design balances two competing objectives: optimizing the outcomes for the subjects in the experiment (``cumulative regret minimization'') and gathering data that will be most useful for policy learning, that is, for learning an assignment rule that will maximize welfare if used after the experiment (``simple regret minimization''). We evaluate alternative experimental designs by collecting pilot data and then conducting a simulation study. Next, we implement our selected algorithm. Finally, we perform a second simulation study anchored to the collected data that evaluates the benefits of the algorithm we chose. Our first result is that the value of a learned policy in this setting is higher when data is collected via a uniform randomization rather than collected adaptively using standard cumulative regret minimization or policy learning algorithms. We propose a simple heuristic for adaptive experimentation that improves upon uniform randomization from the perspective of policy learning at the expense of increasing cumulative regret relative to alternative bandit algorithms. The heuristic modifies an existing contextual bandit algorithm by (i) imposing a lower bound on assignment probabilities that decay slowly so that no arm is discarded too quickly, and (ii) after adaptively collecting data, restricting policy learning to select from arms where sufficient data has been gathered.

==> tables/average_covariate_per_region.tex <==
\begin{tabular}{llrrrr}
\toprule
         &     &    blm &  green &    nra &  planned \\
\midrule
male & mean &  0.412 &  0.454 &  0.535 &    0.504 \\
         & sem &  0.023 &  0.023 &  0.024 &    0.045 \\
white & mean &  0.720 &  0.776 &  0.895 &    0.880 \\
         & sem &  0.021 &  0.019 &  0.015 &    0.029 \\
last\_donation & mean &  2.076 &  2.029 &  1.986 &    2.160 \\
         & sem &  0.046 &  0.045 &  0.046 &    0.085 \\
religious\_spiritual & mean &  0.501 &  0.676 &  0.719 &    0.608 \\
         & sem &  0.023 &  0.021 &  0.022 &    0.044 \\
rural & mean &  0.742 &  0.697 &  0.810 &    0.768 \\
         & sem &  0.020 &  0.021 &  0.019 &    0.038 \\
political\_leaning & mean &  2.766 &  3.616 &  5.323 &    4.232 \\
         & sem &  0.074 &  0.089 &  0.077 &    0.167 \\
age & mean & 43.918 & 49.680 & 49.286 &   45.624 \\
         & sem &  0.802 &  0.748 &  0.801 &    1.446 \\
views\_right\_bear\_arms & mean &  4.171 &  4.216 &  1.334 &    1.432 \\
         & sem &  0.039 &  0.037 &  0.023 &    0.044 \\
views\_global\_warming & mean &  4.293 &  4.216 &  2.735 &    5.000 \\
         & sem &  0.043 &  0.045 &  0.053 &    0.000 \\
views\_abortion & mean &  2.028 &  2.876 &  3.270 &    2.432 \\
         & sem &  0.060 &  0.070 &  0.073 &    0.155 \\
views\_immigration & mean &  2.334 &  4.521 &  4.346 &    4.024 \\
         & sem &  0.036 &  0.023 &  0.048 &    0.114 \\
news\_fox & mean &  2.134 &  3.106 &  3.368 &    2.928 \\
         & sem &  0.076 &  0.089 &  0.092 &    0.171 \\
news\_cnn & mean &  3.013 &  3.083 &  1.938 &    2.560 \\
         & sem &  0.085 &  0.085 &  0.069 &    0.151 \\
news\_wsj & mean &  2.098 &  2.095 &  1.773 &    1.720 \\
         & sem &  0.070 &  0.073 &  0.064 &    0.121 \\
\bottomrule
\end{tabular}


==> tables/contrast_estimates.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Diff. estimate &  Std. Error &  p-value \\
Contrast                   &                 &             &          \\
\midrule
learned\_tree-learned\_fixed &           0.966 &       0.300 &    0.001 \\
\bottomrule
\end{tabular}


==> tables/overlap.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Uniform + Learning phases &  Evaluation phase \\
bandit            &                            &                   \\
\midrule
BootstrapThompson &                      0.159 &             0.267 \\
TreeBagging(50)   &                      0.160 &             0.266 \\
Uniform           &                      0.100 &             0.259 \\
\bottomrule
\end{tabular}


==> tables/pilot_arm_values.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} & \multicolumn{2}{l}{sample mean} & \multicolumn{2}{l}{AIPW[none]} & \multicolumn{2}{l}{AIPW[macf]} & \multicolumn{2}{l}{AIPW[lasso-tlearner]} \\
{} &         avg & stderr &       mean &   sem &       mean &   sem &                 mean &   sem \\
\midrule
aipac      &      -0.159 &  0.376 &     -0.159 & 0.376 &     -0.144 & 0.373 &               -0.193 & 0.364 \\
blm        &       2.027 &  0.439 &      2.027 & 0.455 &      1.809 & 0.387 &                1.682 & 0.375 \\
clinton    &      -0.285 &  0.428 &     -0.285 & 0.428 &     -0.347 & 0.391 &               -0.382 & 0.399 \\
colin      &       1.850 &  0.457 &      1.850 & 0.468 &      2.008 & 0.402 &                2.004 & 0.393 \\
green      &       4.985 &  0.334 &      4.985 & 0.439 &      4.889 & 0.309 &                4.716 & 0.316 \\
nra        &      -2.627 &  0.453 &     -2.627 & 0.476 &     -2.441 & 0.417 &               -2.505 & 0.367 \\
peta       &       1.285 &  0.405 &      1.285 & 0.411 &      1.346 & 0.387 &                1.361 & 0.387 \\
planned    &       4.199 &  0.419 &      4.199 & 0.490 &      3.967 & 0.375 &                3.846 & 0.374 \\
salvation  &       4.917 &  0.373 &      4.917 & 0.466 &      5.004 & 0.377 &                4.821 & 0.372 \\
zuckerberg &       2.829 &  0.354 &      2.829 & 0.388 &      2.793 & 0.344 &                2.750 & 0.352 \\
\bottomrule
\end{tabular}


==> tables/pilot_contrasts.tex <==
\begin{tabular}{llrrrrrrl}
\toprule
{} &                              policy &  len\_scores &  estimate &  stderr &  tstat &  pvalues &  power & hypothesis \\
\midrule
0 &            green-learned\_tree[none] &        1365 &    -1.288 &   0.443 & -2.905 &    0.004 &  1.000 &  two-sided \\
1 &            green-learned\_tree[macf] &        1365 &    -1.273 &   0.463 & -2.752 &    0.006 &  1.000 &  two-sided \\
2 &  green-learned\_tree[lasso-tlearner] &        1365 &    -1.375 &   0.472 & -2.913 &    0.004 &  1.000 &  two-sided \\
\bottomrule
\end{tabular}


==> tables/pilot_covariate_difference.tex <==
\begin{tabular}{llrrr}
\toprule
         &                   &  difference &  stderr &  p-values \\
\midrule
age & planned - green &     -10.824 &   1.160 &     0.000 \\
         & salvation - green &      -3.897 &   1.237 &     0.000 \\
gender & planned - green &      -0.033 &   0.039 &     0.404 \\
         & salvation - green &      -0.046 &   0.041 &     0.262 \\
race & planned - green &       0.447 &   0.036 &     0.000 \\
         & salvation - green &       0.693 &   0.032 &     0.000 \\
marital & planned - green &       0.171 &   0.037 &     0.000 \\
         & salvation - green &      -0.083 &   0.037 &     0.030 \\
last\_charity & planned - green &      -0.037 &   0.062 &     0.549 \\
         & salvation - green &      -0.148 &   0.064 &     0.021 \\
socialMedia & planned - green &       0.212 &   0.097 &     0.020 \\
         & salvation - green &       0.078 &   0.102 &     0.405 \\
political\_leanings\_1 & planned - green &      -0.535 &   0.131 &     0.000 \\
         & salvation - green &       1.372 &   0.137 &     0.000 \\
whichReligion0 & planned - green &      -0.235 &   0.038 &     0.000 \\
         & salvation - green &       0.118 &   0.041 &     0.002 \\
whichReligion1 & planned - green &       0.261 &   0.033 &     0.000 \\
         & salvation - green &      -0.077 &   0.030 &     0.026 \\
whichReligion2 & planned - green &      -0.021 &   0.036 &     0.545 \\
         & salvation - green &      -0.029 &   0.037 &     0.428 \\
whichReligion3 & planned - green &      -0.005 &   0.016 &     0.719 \\
         & salvation - green &      -0.012 &   0.016 &     0.443 \\
howReligion & planned - green &      -0.258 &   0.038 &     0.000 \\
         & salvation - green &       0.055 &   0.041 &     0.154 \\
locality & planned - green &      -0.004 &   0.036 &     0.895 \\
         & salvation - green &      -0.103 &   0.036 &     0.004 \\
views\_right\_bear\_arms & planned - green &       0.094 &   0.134 &     0.479 \\
         & salvation - green &      -1.103 &   0.132 &     0.000 \\
views\_global\_warming & planned - green &      -0.468 &   0.116 &     0.000 \\
         & salvation - green &       1.165 &   0.130 &     0.000 \\
views\_abortion & planned - green &      -2.052 &   0.134 &     0.000 \\
         & salvation - green &       1.516 &   0.142 &     0.000 \\
views\_immigration & planned - green &       0.357 &   0.132 &     0.006 \\
         & salvation - green &      -0.979 &   0.132 &     0.000 \\
news\_fox & planned - green &      -0.367 &   0.109 &     0.001 \\
         & salvation - green &       0.600 &   0.122 &     0.000 \\
news\_cnn & planned - green &      -0.261 &   0.116 &     0.019 \\
         & salvation - green &      -0.713 &   0.120 &     0.000 \\
news\_wp & planned - green &       0.245 &   0.109 &     0.018 \\
         & salvation - green &      -0.607 &   0.112 &     0.000 \\
news\_wsj & planned - green &       0.266 &   0.095 &     0.005 \\
         & salvation - green &      -0.063 &   0.097 &     0.523 \\
\bottomrule
\end{tabular}


==> tables/pilot_fixed_policy_value.tex <==
\begin{tabular}{llrrrr}
\toprule
{} &                        policy &  len\_scores &  estimate &  stderr &  tstat \\
\midrule
0 &            learned\_tree[none] &        1365 &     6.730 &   0.417 & 16.126 \\
1 &            learned\_tree[macf] &        1365 &     6.069 &   0.385 & 15.779 \\
2 &  learned\_tree[lasso-tlearner] &        1365 &     6.486 &   0.381 & 17.025 \\
3 &                       planned &        1365 &     5.126 &   0.360 & 14.251 \\
4 &                         green &        1365 &     5.126 &   0.360 & 14.251 \\
\bottomrule
\end{tabular}


==> tables/pilot_heterogeneity.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{3}{l}{planned-green} & \multicolumn{3}{l}{salvation-green} \\
{} &    difference & stderr & p-values &      difference & stderr & p-values \\
\midrule
age                   &        -5.668 &  1.068 &    0.000 &           4.465 &  1.796 &    0.035 \\
gender                &         0.068 &  0.052 &    0.191 &           0.096 &  0.081 &    0.238 \\
race                  &         0.019 &  0.046 &    0.679 &          -0.000 &  0.000 &    0.265 \\
marital               &         0.098 &  0.051 &    0.060 &          -0.048 &  0.073 &    0.481 \\
last\_charity          &         0.149 &  0.087 &    0.069 &          -0.120 &  0.119 &    0.343 \\
socialMedia           &        -0.089 &  0.102 &    0.425 &          -0.261 &  0.170 &    0.183 \\
political\_leanings\_1  &        -1.562 &  0.121 &    0.000 &           2.292 &  0.179 &    0.000 \\
whichReligion0        &        -0.080 &  0.047 &    0.071 &           0.433 &  0.067 &    0.000 \\
whichReligion1        &         0.202 &  0.048 &    0.000 &          -0.280 &  0.077 &    0.000 \\
whichReligion2        &        -0.112 &  0.050 &    0.016 &          -0.106 &  0.079 &    0.143 \\
whichReligion3        &        -0.010 &  0.021 &    0.606 &          -0.047 &  0.042 &    0.095 \\
howReligion           &        -0.129 &  0.050 &    0.005 &           0.362 &  0.072 &    0.000 \\
locality              &        -0.043 &  0.049 &    0.362 &          -0.059 &  0.070 &    0.358 \\
views\_right\_bear\_arms &         1.279 &  0.159 &    0.000 &          -2.046 &  0.290 &    0.000 \\
views\_global\_warming  &        -0.007 &  0.130 &    0.958 &           2.027 &  0.150 &    0.000 \\
views\_abortion        &        -0.436 &  0.080 &    0.000 &           1.652 &  0.063 &    0.000 \\
views\_immigration     &         0.848 &  0.181 &    0.000 &          -1.870 &  0.260 &    0.000 \\
news\_fox              &        -0.388 &  0.138 &    0.002 &           0.977 &  0.202 &    0.000 \\
news\_cnn              &        -0.068 &  0.151 &    0.639 &          -0.886 &  0.204 &    0.000 \\
news\_wp               &         0.253 &  0.144 &    0.065 &          -0.743 &  0.216 &    0.000 \\
news\_wsj              &        -0.133 &  0.140 &    0.299 &          -0.363 &  0.200 &    0.057 \\
\bottomrule
\end{tabular}


==> tables/pilot_learned_tree_value.tex <==
\begin{tabular}{lllll}
\toprule
{} & len\_scores & estimate & stderr &  tstat \\
policy                       &            &          &        &        \\
\midrule
learned\_tree[none]           &       1365 &    7.596 &  0.709 & 10.707 \\
learned\_tree[macf]           &       1365 &    6.069 &  0.385 & 15.779 \\
learned\_tree[lasso-tlearner] &       1365 &    6.278 &  0.377 & 16.638 \\
\bottomrule
\end{tabular}


==> tables/pilot_proportions.tex <==
\begin{tabular}{lllll}
\toprule
{} &  Mean & Std. Error & t-stat & p-value \\
\midrule
aipac      & 0.108 &      0.006 &  1.416 &   0.157 \\
blm        & 0.093 &      0.006 & -1.184 &   0.237 \\
clinton    & 0.100 &      0.006 &  0.064 &   0.949 \\
colin      & 0.098 &      0.006 & -0.387 &   0.699 \\
green      & 0.100 &      0.006 &  0.000 &   1.000 \\
nra        & 0.102 &      0.006 &  0.379 &   0.705 \\
peta       & 0.103 &      0.006 &  0.504 &   0.614 \\
planned    & 0.090 &      0.005 & -1.804 &   0.071 \\
salvation  & 0.102 &      0.006 &  0.316 &   0.752 \\
zuckerberg & 0.103 &      0.006 &  0.504 &   0.614 \\
\bottomrule
\end{tabular}


==> tables/policy_values.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Value estimate &  Std. Error \\
Policy        &                 &             \\
\midrule
learned\_tree  &           6.619 &       1.523 \\
learned\_tree2 &           5.471 &       1.499 \\
learned\_fixed &           2.573 &       1.506 \\
\bottomrule
\end{tabular}


==> tables/pooled_simulation_learned_policy_value.tex <==
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
Regularization &   5 &   10 &   20 &   40 &   50 &   80 &   100 &   160 &   320 &   500 &   640 &   1280 &   2560 \\
\midrule
Uniform               &   5.88 &    5.85 &    5.86 &    5.84 &    5.84 &    5.84 &     5.83 &     5.79 &     5.76 &     5.74 &     5.69 &      5.61 &      5.52 \\
         &   0.02 &    0.02 &    0.02 &    0.02 &    0.02 &    0.02 &     0.02 &     0.02 &     0.02 &     0.02 &     0.02 &      0.02 &      0.02 \\
TreeBagging(50)    &   5.92 &    5.89 &    5.90 &    5.89 &    5.92 &    5.89 &     5.89 &     5.84 &     5.80 &     5.75 &     5.74 &      5.69 &      5.55 \\
 &   0.02 &    0.02 &    0.02 &    0.02 &    0.02 &    0.02 &     0.02 &     0.02 &     0.02 &     0.02 &     0.02 &      0.01 &      0.02 \\
 BootstrapThompson    &   5.83 &    5.83 &    5.84 &    5.82 &    5.81 &    5.82 &     5.81 &     5.79 &     5.75 &     5.71 &     5.69 &      5.60 &      5.51 \\
&   0.02 &    0.02 &    0.02 &    0.02 &    0.02 &    0.02 &     0.02 &     0.02 &     0.02 &     0.02 &     0.02 &      0.02 &      0.02 \\

BootstrapES            &   5.83 &    5.83 &    5.85 &    5.79 &    5.82 &    5.81 &     5.81 &     5.77 &     5.74 &     5.73 &     5.69 &      5.58 &      5.51 \\
      &   0.02 &    0.02 &    0.02 &    0.02 &    0.02 &    0.02 &     0.02 &     0.02 &     0.02 &     0.02 &     0.02 &      0.02 &      0.02 \\
BootstrapTTTS        &   5.83 &    5.86 &    5.83 &    5.81 &    5.82 &    5.83 &     5.83 &     5.81 &     5.74 &     5.75 &     5.68 &      5.61 &      5.49 \\
   &   0.02 &    0.02 &    0.02 &    0.02 &    0.02 &    0.02 &     0.02 &     0.02 &     0.02 &     0.02 &     0.02 &      0.02 &      0.02 \\

Improvement                          & 100.76 &  100.78 &  100.60 &  100.82 &  101.34 &  100.79 &   101.00 &   100.90 &   100.67 &   100.13 &   100.77 &    101.42 &    100.67 \\
\multicolumn{14}{l}{(TreeBagging(50) as \% of Uniform)}\\ 
\bottomrule
\end{tabular}


==> tables/pooled_simulation_regret.tex <==
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
Regularization &   5 &   10 &   20 &   40 &   50 &   80 &   100 &   160 &   320 &   500 &   640 &   1280 &   2560 \\
\midrule
Uniform             &   4.83 &    4.77 &    4.76 &    4.75 &    4.73 &    4.67 &     4.65 &     4.57 &     4.48 &     4.37 &     4.31 &      4.09 &      3.80 \\
        &   0.01 &    0.01 &    0.01 &    0.01 &    0.01 &    0.01 &     0.01 &     0.01 &     0.01 &     0.01 &     0.01 &      0.01 &      0.01 \\
TreeBagging(50)       &   3.84 &    3.80 &    3.78 &    3.75 &    3.72 &    3.69 &     3.67 &     3.61 &     3.55 &     3.44 &     3.39 &      3.21 &      2.99 \\
  &   0.01 &    0.01 &    0.01 &    0.01 &    0.01 &    0.01 &     0.01 &     0.01 &     0.01 &     0.01 &     0.01 &      0.01 &      0.01 \\
BootstrapThompson     &   3.67 &    3.64 &    3.61 &    3.60 &    3.58 &    3.55 &     3.53 &     3.47 &     3.38 &     3.31 &     3.27 &      3.10 &      2.92 \\
&   0.01 &    0.01 &    0.01 &    0.01 &    0.01 &    0.01 &     0.01 &     0.01 &     0.01 &     0.01 &     0.01 &      0.01 &      0.01 \\

BootstrapES           &   3.80 &    3.75 &    3.76 &    3.73 &    3.71 &    3.67 &     3.65 &     3.59 &     3.53 &     3.45 &     3.40 &      3.23 &      3.04 \\
     &   0.01 &    0.01 &    0.01 &    0.01 &    0.01 &    0.01 &     0.01 &     0.01 &     0.01 &     0.01 &     0.01 &      0.01 &      0.01 \\
BootstrapTTTS         &   3.79 &    3.75 &    3.75 &    3.73 &    3.71 &    3.67 &     3.64 &     3.57 &     3.52 &     3.44 &     3.39 &      3.23 &      3.04 \\
    &   0.01 &    0.01 &    0.01 &    0.01 &    0.01 &    0.01 &     0.01 &     0.01 &     0.01 &     0.01 &     0.01 &      0.01 &      0.01 \\

Reduction                           &  79.41 &   79.72 &   79.49 &   78.96 &   78.82 &   79.01 &    78.96 &    78.89 &    79.16 &    78.86 &    78.69 &     78.50 &     78.73 \\
\multicolumn{14}{l}{(TreeBagging(50) as \% of Uniform)}\\ 
\bottomrule
\end{tabular}


==> tables/post_simulation_learned_policy_value_reg500.tex <==
\begin{tabular}{llrrrr}
\toprule
        & Mean &  Std. Error & Improvement (\% of Uniform)\\
Bandit & {} &               & \\
\midrule
Uniform & 5.645 &     0.001 & \\
TreeBagging(50) & 5.691 &      0.001 & 100.81\\
\bottomrule
\end{tabular}

